Zero-Gated Language-conditioned Human Motion Prediction

Pose histories provide the core kinematic evidence for 3D human motion prediction, but they lack explicit high-level semantic guidance. This paper introduces ZGL, a lightweight language-conditioned predictor that uses captions of the observed motion as a semantic prior while preserving a strong motion backbone as the main source of dynamics. We render only the observed poses, generate a one-sentence description with a vision-language model, encode the caption with a frozen CLIP-L text tower, and project it into a small set of conditioning tokens. These tokens are injected into a DCT-based spatial-temporal Transformer by compact crossattention adapters with zero gates: each adapter output is multiplied by a learnable gate initialized to zero, so the full network is numerically identical to the pose-only baseline at initialization and can learn to use language only when it reduces prediction error. On Human3.6M, ZGL improves overall MPJPE over representative motion-prediction baselines in our comparison. Results on CMUMocap further show that compact caption conditioning transfers to a second benchmark and provides a practical semantic cue for 3D human motion prediction.

==> sections/02_related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{3D Human Motion Prediction.}
Modern HMP largely descends from sequence-to-sequence
recurrent models~\cite{martinez2017human} and has since converged on
two strong architectural families: graph and temporal convolutional
networks~\cite{mao2019learning, dang2021msr}, and transformer
backbones with parallel spatial--temporal attention. The siMLPe
family~\cite{guo2023back} demonstrates that very lightweight MLPs
operating in the DCT domain are competitive when paired with the
right loss schedule, which we adopt as our baseline. We work on
Human3.6M~\cite{ionescu2014h36m} and CMU Mocap, two common benchmarks
reported by recent state-of-the-art motion prediction work.

\paragraph{Text-conditioned motion modelling.}
Text-to-motion \emph{generation} -- producing a full motion sequence
from a caption alone -- has matured rapidly. MotionDiffuse
\cite{zhang2022motiondiffuse} and MDM~\cite{tevet2022mdm} establish
diffusion-based generators; MoMask~\cite{guo2024momask} and
T2M-GPT~\cite{zhang2023t2mgpt} adopt VQ-VAE representations with
masked or autoregressive decoders. SALAD~\cite{hong2025salad}
introduces skeleton-aware latent diffusion and per-word, per-joint
attention maps. These models reliably benefit from text because text
is the dominant signal.

\paragraph{Text in motion \emph{prediction}.}
The situation in HMP is less clear-cut: the past pose history is itself
a strong action predictor, so text is at best a complementary prior.
For this reason, our work focuses on a compact conditioning interface
that keeps the motion backbone central. We ask whether a single
cross-attention adapter per encoder block, together with careful choices
of injection location, capacity, and dropout, is enough to use caption
semantics effectively.

\paragraph{Cross-attention adapters with zero-init gates.}
The use of an additive cross-attention adapter with a zero-initialised
gate is widespread in image generation
(LayerScale~\cite{touvron2021going}, DiT~\cite{peebles2023dit},
PixArt-$\alpha$~\cite{chen2023pixart}) and in vision-language
modelling (Flamingo gated cross-attention
\cite{alayrac2022flamingo}). The shared principle -- step-0 forward
is the identity, so any improvement is attributable to the adapter --
is exactly what we want for a clean text-vs-no-text ablation. We are,
to the best of our knowledge, the first to apply this primitive
systematically to 3D human motion prediction.


==> tables/cross_dataset.tex <==
\begin{table}[H]
  \centering
  \caption{\textbf{Cross-dataset transfer.} Lower is better.}
  \label{tab:cross}
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}llrrr@{}}
    \toprule
    Dataset & Method & short-AVG & long-AVG & \textbf{Total-AVG}\\
    \midrule
    \multirow{2}{*}{H3.6M}
        & B0 baseline (no text) & 33.33 & 93.63 & 53.43 \\
        & + text (ours)         & \textbf{32.83} & \textbf{92.56} & \textbf{52.74} \\
    \midrule
    \multirow{2}{*}{CMU Mocap}
        & B0 baseline (no text) & 20.03 & 66.81 & 35.63 \\
        & + text (ours)         & \textbf{19.42} & \textbf{65.89} & \textbf{34.91} \\
    \bottomrule
  \end{tabular}
\end{table}

